Improving and Expanding Video Editing Capabilities Without Videos

Image editing models can follow a wide range of instructions, but video editing models still lag behind, limited in part by the difficulty of collecting paired source and edited videos. Is it possible to transfer advanced image editing capabilities to video editors without new paired videos? We introduce Image-to-Video Transfer (I2VT), which improves pretrained video editors and expands them to new editing tasks using an image editor. It enables efficient post-training with no architectural changes and no new videos, using only individual images. Our key idea is to let the video editor role-play as an image editor: it edits an image as a one-frame video, with the image editor guiding the video editor's predictions at each denoising step. Although the video editor sees only single images during training, at test time it applies the improved and expanded capabilities to whole video clips while preserving temporal consistency. To push the boundaries of video editing, we introduce OpenVE++, an extension of OpenVE-Bench that adds four new editing tasks useful for video production, including action changes, expression changes, body movements, and scene relighting. Our experiments across three different video editors show that I2VT improves existing editing capabilities and expands them to new tasks, and our models achieve state-of-the-art (SOTA) performance on both OpenVE-Bench and OpenVE++.

==> sections/0_abstract.tex <==
Image editing models can follow a wide range of instructions, but video editing models still lag behind, limited in part by the difficulty of collecting paired source and edited videos.
Is it possible to transfer advanced image editing capabilities to video editors without new paired videos?
We introduce Image-to-Video Transfer (\textbf{\methodname}\unskip), which improves pretrained video editors and expands them to new editing tasks using an image editor. It enables efficient post-training with no architectural changes and no new videos, using only individual images.
Our key idea is to let the video editor \emph{role-play as an image editor}: it edits an image as a \emph{one-frame video}, with the image editor guiding the video editor's predictions at each denoising step.
Although the video editor sees only single images during training, at test time it applies the improved and expanded capabilities to whole video clips while preserving temporal consistency.
To push the boundaries of video editing, we introduce \textbf{OpenVE++}, an extension of OpenVE-Bench that adds four new editing tasks useful for video production, including \emph{action changes}, \emph{expression changes}, \emph{body movements}, and \emph{scene relighting}.
Our experiments across three different video editors show that \ours improves existing editing capabilities and expands them to new tasks, and our models achieve state-of-the-art (SOTA) performance on both OpenVE-Bench and \benchname.


==> sections/1_introduction.tex <==
\section{Introduction}
\label{sec:intro}

\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{figures/method_motivation.pdf}
\vspace{-1.2em}
\caption{\textbf{Motivation and intuition.} Left: image editors handle complex edits such as actions and relighting on single frames, whereas video editors lack the paired data to learn them. Our goal is a video editor that makes these edits while keeping the video temporally consistent.
Middle: can a video editor learn to edit images by treating each image as a one-frame video? Right: video editing ability improves while temporal quality remains comparable.}
\label{fig:motivation}

\end{figure*}

Recent image editing models have advanced rapidly and can follow detailed instructions and offer fine-grained control over a wide range of edits~\citep{openai2025gpt4oimage,google2025nanobananapro,labs2025kontext,wu2025qwenimage,zhang2025icedit,deng2025bagel,bfl2025flux2,seedream2025seedream4,seed2026seedream5pro}.
This progress has been supported by increasingly diverse image editing datasets~\citep{brooks2023instructpix2pix,zhang2023magicbrush,zhao2024ultraedit,yu2025anyedit,wei2025omniedit}.
However, current video editors~\citep{cheng2024insv2v,wu2025insvie,zi2025senorita,hu2025vivid10m,bai2026ditto,he2025openve} still perform only moderately well on basic edit types such as object removal. They struggle even more with edits that change a person's actions, facial expressions, body movements, or a scene's lighting, although video production often needs these edits~\citep{burgert2026motionv2v,papantoniou2022ned,zhang2025scaling,zhou2025lightavideo,fang2025relightvid} (\Cref{fig:motivation}, left).

This gap remains even though modern image and video editors are built in similar ways: they use the same flow-matching objective and similar diffusion transformer (DiT) architectures~\citep{peebles2023dit}, and many recent models also share a variational autoencoder (VAE)~\citep{kingma2013vae} latent space~\citep{song2026joyaiimage,wu2025qwenimage,bernini2026bernini,yang2025videocof}.
One reason video editors still lag behind is training data. A good training pair for video editing must include an edited video that follows the instruction closely over the whole clip while leaving unrelated regions unchanged. Yet current data pipelines struggle to produce such videos, especially when edits become complex and diverse~\citep{bai2026ditto,burgert2026motionv2v,pan2026nova}.
This raises a question: \emph{can a video editor improve its existing editing capabilities and expand them to new tasks \textbf{without} new paired videos?}

To answer this question, we introduce Image-to-Video Transfer (\textbf{\methodname}\unskip), which efficiently improves and expands a pretrained video editor using only images instead of new paired videos.
Our intuition is that an image is simply a one-frame video, so editing images well could be a foundation for editing videos well.
We therefore let the video editor \emph{role-play as an image editor}: it edits a source image as a \emph{one-frame video} under the supervision of a frozen image editor.
A direct way to give this supervision is offline distillation, which fine-tunes the video editor on the image editor's pre-computed edit results. \methodname instead lets the image editor tell the video editor how to update its current noisy prediction at each step of its own denoising trajectory (\Cref{fig:pipeline}).
Although the video editor sees only single images during training, at test time it applies the improved and expanded capabilities to whole video clips while preserving temporal consistency (\Cref{fig:teaser}).

To push the boundaries of video editing, we introduce \textbf{\benchname}, an extension of OpenVE-Bench~\citep{he2025openve} that adds four editing tasks useful for video production: \textit{Action Change}, \textit{Expression Change}, \textit{Body Movement}, and \textit{Scene Relighting} (\Cref{fig:benchmark_data}). These tasks test whether video editors can change a person's performance and a scene's lighting, which video production often requires~\citep{burgert2026motionv2v,papantoniou2022ned,zhou2025lightavideo}.
Across three video editors, our experiments show that \methodname improves basic edits and enables new tasks that their pretrained base editors barely perform, and the resulting models achieve state-of-the-art (SOTA) results among the open-source video editors we compare.
Our contributions are as follows:
\begin{list}{$\bullet$}{%
    \setlength{\leftmargin}{1.2em}%
    \setlength{\labelwidth}{0.8em}%
    \setlength{\labelsep}{0.4em}%
    \setlength{\itemsep}{0.2em}%
    \setlength{\topsep}{0.2em}%
}
    \item We propose \methodname, which improves and expands pretrained video editors by letting them role-play as image editors, without new paired videos or architecture changes.
    \item We introduce \benchname\unskip, an extension of OpenVE-Bench that adds four new editing tasks useful for video production: action changes, expression changes, body movements, and scene relighting.
    \item We validate \methodname across three video editing models: editing capabilities improved and expanded with single images generalize to whole video clips while preserving temporal consistency, and the resulting models achieve SOTA results on OpenVE-Bench and \benchname.
\end{list}


==> sections/2_related_work.tex <==
\section{Related Work}
\label{sec:related}

\paragraph{Instruction-Based Video Editing.}
Early video editors adapt a text-to-image or text-to-video prior at inference time without paired editing data, through inversion~\citep{mokady2023nulltext,qi2023fatezero,liu2024videop2p,ceylan2023pix2video,cohen2024slicedit}, attention control and sharing across frames~\citep{hertz2022prompt,khachatryan2023text2videozero,zhang2023controlvideo,kara2024rave,li2024vidtome,jeong2024groundavideo,yang2025videograin}, or feature propagation~\citep{geyer2023tokenflow,yang2023rerender,cong2024flatten,yang2024fresco,wang2024cove}, and some tune the model or a video representation on each source video~\citep{wu2023tuneavideo,chai2023stablevideo,ouyang2024codef}. Learning-based editors instead fine-tune a pretrained video backbone~\citep{wan2025wan,kong2024hunyuanvideo,yang2024cogvideox,hacohen2024ltxvideo} on synthetic source, instruction, and target triplets~\citep{cheng2024insv2v,wu2025insvie,zi2025senorita,hu2025vivid10m,bai2026ditto,he2025openve,zhang2026sama,yang2025videocof,liao2025icve,zhou2026thinkv2v} or attach task adapters to it~\citep{jiang2025vace}, and recent unified models combine generation and editing across modalities~\citep{wei2025univideo,ju2025editverse,tan2026omnivideo,chen2026vino,pan2026omniweaving,lin2026kiwiedit,loomvideo2026,mou2025instructx,liu2026tide,huang2026jova}.

Image editors also help construct paired training videos by editing a source frame and using a video model to generate the edited clip~\citep{bai2026ditto,bernini2026bernini,wang2026live}.
However, training data still concentrate on basic edit types such as object addition, removal, replacement, and style transfer~\citep{bai2026ditto,he2025openve}, while reliably changing a subject's actions, expressions, or body movements remains difficult.

\paragraph{Image Editing for Video Editing.}
Paired image editing data are far more abundant than paired video edits~\citep{brooks2023instructpix2pix,zhang2023magicbrush,zhao2024ultraedit,yu2025anyedit,wei2025omniedit}, and many prior works bring them to video.
One group edits the first frame with an image editor and fine-tunes an image-to-video (I2V) or video diffusion model to propagate the edit, either on each source video~\citep{ouyang2024i2vedit} or by training added modules on videos~\citep{pan2026nova,seo2026propfly,lei2026editdistill}.
Another group trains on image editing pairs by repeating frames or warping them into synthetic motion~\citep{wang2026live,zhang2026flowmimic}, uses image edit pairs as in-context examples~\citep{qu2026vincienext}, or mixes image and video training in unified editors~\citep{xia2025dreamve,ju2025editverse,wei2025univideo,rao2026insedit,chen2026vino,mai2025easyv2v}.
A third group modifies the architecture of pretrained image or video generative models, or adds adapters to them, to enable video editing~\citep{singer2024eve,xu2026imvideoedit,yu2026vifeedit,bai2026qwenvideoedit}.
In contrast, \methodname fine-tunes an existing video editor directly on single source images along its own denoising trajectory, as in on-policy distillation~\citep{ross2011dagger,agarwal2024gkd,fang2026flowopd,li2026diffusionopdunifiedperspectiveonpolicy,zhou2026danceopd,li2026cfgopd}, without constructing video targets, engineering artificial motion, or altering the core architecture.


==> sections/3_method.tex <==
\section{Method}
\label{sec:method}

\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{figures/method_pipeline.pdf}
\vspace{-0.9em}
\caption{\textbf{\methodname and the offline distillation baseline.}
Left: offline distillation fine-tunes on teacher-edited images. Middle: \methodname supervises the student along its own rollout. The cross marks stop-gradient.
Right: at inference, the student edits whole video clips.}
\label{fig:pipeline}

\end{figure*}

Image-to-Video Transfer (\methodname\unskip) lets a pretrained video editor \emph{role-play as an image editor}: it edits an individual image as a \emph{one-frame video}, with a frozen image editor guiding its predictions at each denoising step.
During fine-tuning, the video student takes one source image and an editing instruction at a time.
\methodname matches the teacher's velocity predictions on the student's own denoising trajectory. As a baseline, we also consider offline distillation, which fine-tunes the student on source and edited image pairs prepared by the image teacher.

\subsection{Preliminaries}
\label{sec:setup}

\noindent\textbf{Latent Diffusion and Flow Matching.}
Latent diffusion models~\citep{rombach2022ldm} use a pretrained variational autoencoder (VAE)~\citep{kingma2013vae} to encode an image into a clean latent $\vx_0$ and decode generated latents back to images.
In flow matching~\citep{lipman2023flow,liu2023rectified}, a noisy latent is constructed as $\vx_t=(1-t)\vx_0+t\epsilon$, where $\epsilon\sim\mathcal{N}(0,I)$ and $t\in[0,1]$, so $\vx_1=\epsilon$ is the noise endpoint.
The model predicts the velocity $\mathrm{d}\vx_t/\mathrm{d}t=\epsilon-\vx_0$, and during sampling its velocity field $\vv(\vx_t,t,c)$ moves the noisy latent $\vx_t$ from noise at $t=1$ toward the clean latent at $t=0$, conditioned on an editing instruction $c$ and the source image.

\noindent\textbf{Image and Video Editors.}
The frozen image teacher $\phi$ and the pretrained video student $\theta$ predict velocities $\phi(\vx_t,t,c_{\mathrm{img}})$ and $\theta(\vx_t,t,c_{\mathrm{video}})$, respectively.
Each example in our training set $\mathcal D$ contains a source image $I_s$, which the student treats as a \emph{one-frame video}, and two instructions, $c_{\mathrm{img}}$ and $c_{\mathrm{video}}$, that describe the same edit.

\subsection{Offline Distillation Baseline}
\label{sec:offline}


Since an image is simply a one-frame video, a good video editor should also edit images well. We therefore first try offline distillation, in which the video editor is fine-tuned on image pairs edited by the image editor. For each training example, the image editor applies the instruction $c_{\mathrm{img}}$ to the source image $I_s$ and produces an edited image $I_e$.
We fine-tune the pretrained video editor on each source and edited image pair $(I_s,I_e)$, treating both images as one-frame videos and using $c_{\mathrm{video}}$ as the editing instruction. To form the flow-matching target, we encode $I_e$ into a clean latent $\vx_0^e$ and add noise at a random time $t$ to obtain $\vx_t^e=(1-t)\vx_0^e+t\epsilon$, where the superscript $e$ denotes the edited target. The student learns to predict the velocity $\epsilon-\vx_0^e$:
\begin{equation}
  \cL_{\mathrm{off}} = \E_{\mathcal D,t,\epsilon}
    \big\lVert \theta(\vx_t^e,t,c_{\mathrm{video}})
    -(\epsilon-\vx_0^e)\big\rVert_2^2.
  \label{eq:sft}
\end{equation}

Offline distillation requires a separate stage in which the teacher generates the edited targets. This offline approach fine-tunes the student on noised teacher outputs rather than states from its own rollouts, which may disrupt the student's original rollout distribution~\citep{agarwal2024gkd,gu2024minillm}.

\begin{figure*}[t]
\centering
\setlength{\abovecaptionskip}{4pt}
\includegraphics[width=\textwidth]{figures/openvepp_composition.pdf}
\caption{\textbf{Editing tasks in \benchname.} Source frames and instructions illustrate the four task groups evaluated across 207 clips.}
\label{fig:benchmark_data}
\end{figure*}

\subsection{\methodname}
\label{sec:opd}


\methodname is designed to fine-tune the video student along its own denoising trajectory with supervision from an image editor: the student edits each source image as a one-frame video from noise, and the teacher guides its prediction at each step.
We take advantage of the shared VAE latent space used by existing image and video models, including JoyAI-Image-Edit, Qwen-Image, Wan2.1, and Wan2.2-14B~\citep{song2026joyaiimage,wu2025qwenimage,wan2025wan,wan2025wan22}, which lets the teacher predict a target velocity directly from the student's noisy latent.

As shown in \Cref{fig:pipeline} (middle), for each training example we initialize the student at $\vx_{t_K}=\epsilon$ with $\epsilon\sim\mathcal{N}(0,I)$ and roll out $K$ denoising steps, $\vx_{t_K}\to\cdots\to\vx_{t_0}$. The timesteps decrease from $t_K=1$ (noise) to $t_0=0$ (the edited image), and each step updates the state as follows:
\begin{equation}
  \vx_{t_{k-1}}
    = \vx_{t_k}+(t_{k-1}-t_k)\,
    \underbrace{\theta(\vx_{t_k},t_k,c_{\mathrm{video}})}_{\text{rollout velocity}}.
  \label{eq:guided-rollout}
\end{equation}
At each step $k$, we feed the state $\vx_{t_k}$ to the teacher, which returns a target velocity for the edited frame, and we fine-tune the student by matching its own velocity to this target:
\begin{equation}
  \cL_{\mathrm{I2VT}}
  = \lVert \underbrace{\theta(\vx_{t_k},t_k,c_{\mathrm{video}})}_{\text{student velocity}}
    - \sg(\underbrace{\phi(\vx_{t_k},t_k,c_{\mathrm{img}})}_{\text{teacher velocity}}) \rVert_2^2,
  \label{eq:loss}
\end{equation}
where $\sg$ is the stop-gradient operator, and we average the loss over the $K$ rollout steps, training examples, and noise samples. Rollout states and teacher targets are treated as constants, so gradients flow only through the student velocity.

\noindent\textbf{Guidance.}
Image and video editors follow the instruction through classifier-free guidance (CFG)~\citep{ho2022cfg}.
For a diffusion model $\theta$ and a guidance scale $\omega$, the guided velocity is
\begin{equation}
  \theta^{\omega}(\vx_t,t,c)
    = (1-\omega)\theta(\vx_t,t,\varnothing)
       +\omega\,\theta(\vx_t,t,c),
  \label{eq:cfg}
\end{equation}
where $\varnothing$ denotes an empty or negative prompt.
In \methodname, the rollout, student, and teacher velocities each use their own scale, $\omega_R$, $\omega_S$, and $\omega_T$.
We set all three to $1$ by default and raise the teacher guidance to $\omega_T=2$ where the student is weak, namely on action changes and body movements and for VideoCoF (\Cref{sec:guidance_scales}). The settings for each model and task are listed in \PaperSupp{}.

\noindent\textbf{Inference.}
At inference time, the teacher is discarded, and the student edits a source video using the sampler and the same settings as the pretrained editor.
Although fine-tuned only on single frames, it generalizes the improved and expanded editing capabilities to the whole video (\Cref{fig:main_new_abilities}).

\subsection{Task and Training Data}
\label{sec:training_data}

We build \textbf{\datasetfull\unskip} by sampling individual frames from OpenVE-3M~\citep{he2025openve}, a dataset already commonly used to train video editors~\citep{lin2026kiwiedit,zhang2026sama}.
We organize these images and their instructions into two pools: the OpenVE pool for basic edits and the \benchname pool for four new task groups. \textit{Action Change} covers head, gaze, and arm edits where the person stays in place, distinct from \textit{Body Movement}, which involves whole-person movements like crouching, jumping, sitting down, standing up, and turning (\Cref{fig:benchmark_data}). \textit{Expression Change} covers facial expressions such as sadness, happiness, and anger, and \textit{Scene Relighting} changes the light type and direction.

For the new tasks, a Vision-Language Model (VLM) describes the source frame so that we can choose a suitable edit and write its instruction.
We accept an instruction only if the frame contains what the edit needs and does not already show the requested change, so raising an arm, for example, requires that arm to be visible and not already raised.
The two instructions specify the same edit, with wording adapted to each model: $c_{\mathrm{img}}$ refers to a single image, while $c_{\mathrm{video}}$ refers to a video and may include temporal requirements such as ``throughout the video.'' This conversion can be automated with simple text replacements.


==> sections/4_experiments.tex <==
\section{Effectiveness of I2VT}
\label{sec:exp}

\begin{figure*}[!t]
\centering
\includegraphics[width=\textwidth]{figures/offline_vs_i2vt.pdf}
\caption{\textbf{Offline versus online distillation with \methodname.} Bernini-R-1.3B on a basic edit from OpenVE-Bench (left) and a body-movement edit from \benchname (right), showing three frames sampled from each video.}
\label{fig:main_basic_comparison}
\end{figure*}

We apply our approach to three pretrained video editors and study three research questions:

\begin{itemize}[leftmargin=*,itemsep=0pt,topsep=2pt]
\item Can \methodname strengthen basic editing capabilities (\Cref{sec:old})?
\item Can \methodname teach video editors new editing tasks using only images (\Cref{sec:new})?
\item How does online distillation compare with offline distillation (\Cref{sec:offline_comparison})?
\end{itemize}




\subsection{Experimental Setup}
\label{sec:eval_setup}
\paragraph{Models and Data.}
We evaluate \methodname on Bernini-R-1.3B~\citep{bernini2026bernini}, Bernini-R-14B, and VideoCoF~\citep{yang2025videocof}, using the powerful image editor JoyAI-Image-Edit~\citep{song2026joyaiimage} as their shared teacher. The teacher and students share the 16-channel Wan 2.1 VAE latent representation~\citep{wan2025wan}, and their detailed architecture descriptions are in \PaperSupp{}.

\paragraph{Training Configuration.}
We fine-tune each base editor for 200 steps with low-rank adaptation (LoRA)~\citep{hu2022lora}, where each \methodname update uses $K=10$ rollout steps per image and a global batch size of $24$, or $48$ when training jointly on both pools. Because training on single frames instead of videos reduces the number of visual tokens and lowers the cost of spatiotemporal attention, fine-tuning takes only 20 A100 GPU-hours for Bernini-R-1.3B and 20--25 B300 GPU-hours for Bernini-R-14B and VideoCoF.

\subsection{Evaluation Benchmarks and Metrics}
\label{sec:evaluation_setting}


\paragraph{\benchname Benchmark.}
\label{sec:openvepp}
Existing video editing benchmarks mainly evaluate basic edit types. Inspired by ImgEdit-Bench~\citep{ye2026imgedit} and GEdit-Bench~\citep{liu2025step1xedit}, we introduce \benchname, which extends OpenVE-Bench with four new categories defined in \Cref{sec:training_data}. \benchname comprises 207 video--instruction pairs across four categories (42--73 per category), keeping category sizes roughly balanced and matching the per-category scale of OpenVE-Bench~\citep{he2025openve}. Each category covers diverse fine-grained edits, and all source videos are strictly disjoint between the training and evaluation splits. \Cref{fig:benchmark_data} illustrates group sizes and examples for these categories.


\paragraph{Metrics.}
Following the OpenVE-Bench protocol~\citep{he2025openve}, we evaluate basic editing on OpenVE-Bench and new abilities on \benchname. Our automatic evaluation combines two complementary dimensions: \textbf{(i) Semantic and visual alignment}, using Gemini 2.5 Pro~\citep{comanici2025gemini25} and Gemini 3.8 Flash to rate instruction compliance, source consistency, and visual quality, and \textbf{(ii) Temporal consistency and motion dynamics}, using widely adopted VBench~\citep{huang2024vbench} metrics (Sec.~\ref{sec:temporal}). Together, they jointly capture editing fidelity and motion execution. We use Gemini 2.5 Pro to score edits before and after fine-tuning and to compare distillation methods, guidance scales, and training losses. For the comparison with existing editors (\Cref{tab:main}), we report scores from Gemini 2.5 Pro on OpenVE-Bench and from both Gemini 2.5 Pro and Gemini 3.8 Flash on \benchname. Evaluation details, Gemini prompts, and a user study validating alignment with human judgments are provided in \PaperSupp{}.

\subsection{Strengthening Existing Abilities}
\label{sec:old}

To verify whether \methodname strengthens existing abilities, we train on the OpenVE pool and evaluate on OpenVE-Bench (\Cref{tab:old}).

\begin{table}[!htb]
\centering
\fontsize{8}{9.5}\selectfont
\renewcommand{\deltasize}{\fontsize{4.5}{5.5}\selectfont}
\setlength{\tabcolsep}{0.8pt}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}>{\hspace{2pt}}lcccccc<{\hspace{2pt}}@{}}
 & \tablehead{Global\\Style$^{\uparrow}$} & \tablehead{Local\\Change$^{\uparrow}$} & \tablehead{Background\\Change$^{\uparrow}$} & \tablehead{Local\\Remove$^{\uparrow}$} & \tablehead{Local\\Add$^{\uparrow}$} & \tablehead{Overall$^{\uparrow}$} \\
\tabheadrule
\multicolumn{7}{@{}>{\hspace{2pt}}l}{\textbf{Bernini-R-1.3B}} \\
Base  & \scoreonly{3.27} & \scoreonly{4.01} & \scoreonly{2.94} & \scoreonly{2.88} & \scoreonly{2.41} & \scoreonly{3.10} \\
\methodname & \scoredelta{\textbf{4.04}}{+0.77} & \scoredelta{\textbf{4.21}}{+0.20} & \scoredelta{\textbf{3.03}}{+0.09} & \scoredelta{\textbf{3.50}}{+0.62} & \scoredelta{\textbf{2.61}}{+0.20} & \scoredelta{\textbf{3.48}}{+0.38} \\
\tabbodyrule
\multicolumn{7}{@{}>{\hspace{2pt}}l}{\textbf{VideoCoF}} \\
Base & \scoreonly{1.31} & \scoreonly{3.59} & \scoreonly{1.55} & \scoreonly{2.48} & \scoreonly{2.50} & \scoreonly{2.29} \\
\methodname & \scoredelta{\textbf{3.61}}{+2.30} & \scoredelta{\textbf{3.89}}{+0.30} & \scoredelta{\textbf{2.73}}{+1.18} & \scoredelta{\textbf{3.19}}{+0.71} & \scoredelta{\textbf{2.51}}{+0.01} & \scoredelta{\textbf{3.19}}{+0.90} \\
\tabbodyrule
\multicolumn{7}{@{}>{\hspace{2pt}}l}{\textbf{Bernini-R-14B}} \\
Base & \scoreonly{4.16} & \scoreonly{4.30} & \scoreonly{3.16} & \scoreonly{2.66} & \scoreonly{2.35} & \scoreonly{3.33} \\
\methodname & \scoredelta{\textbf{4.41}}{+0.25} & \scoredelta{\textbf{4.55}}{+0.25} & \scoredelta{\textbf{3.24}}{+0.08} & \scoredelta{\textbf{3.45}}{+0.79} & \scoredelta{\textbf{2.76}}{+0.41} & \scoredelta{\textbf{3.68}}{+0.35} \\
\end{tabular*}
\caption{\textbf{Basic edits after distillation.} I2VT raises the basic-edit score of all three video editors.}
\label{tab:old}
\end{table}


\methodname \textbf{improves overall basic editing performance} for all three editors (\Cref{tab:old,fig:basic_edit_types}), raising their scores from $3.10$ to $3.48$, $2.29$ to $3.19$, and $3.33$ to $3.68$. Gains vary across categories: VideoCoF's Local Add score is nearly unchanged ($2.50$ to $2.51$), although its overall score approaches that of base Bernini-R-14B ($3.33$).

\subsection{Adding New Abilities}
\label{sec:new}

To test whether \methodname transfers new editing abilities to video editors, we train on the \textit{Action Change}, \textit{Expression Change}, and \textit{Body Movement} data of the \benchname pool.

\begin{table}[!htb]
\centering
\fontsize{8}{9.5}\selectfont
\renewcommand{\deltasize}{\fontsize{4.5}{5.5}\selectfont}
\setlength{\tabcolsep}{0.8pt}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}>{\hspace{2pt}}lcccc<{\hspace{2pt}}@{}}
 & \tablehead{Action\\Change$^{\uparrow}$} & \tablehead{Expression\\Change$^{\uparrow}$} & \tablehead{Body\\Movement$^{\uparrow}$} & \tablehead{Overall$^{\uparrow}$} \\
\tabheadrule
\multicolumn{5}{@{}>{\hspace{2pt}}l}{\textbf{Bernini-R-1.3B}} \\
Base  & \scoreonly{1.83} & \scoreonly{2.00} & \scoreonly{1.14} & \scoreonly{1.66} \\
\methodname & \scoredelta{\textbf{3.21}}{+1.38} & \scoredelta{\textbf{3.58}}{+1.58} & \scoredelta{\textbf{2.18}}{+1.04} & \scoredelta{\textbf{2.99}}{+1.33} \\
\tabbodyrule
\multicolumn{5}{@{}>{\hspace{2pt}}l}{\textbf{VideoCoF}} \\
Base & \scoreonly{1.21} & \scoreonly{1.26} & \scoreonly{1.04} & \scoreonly{1.17} \\
\methodname & \scoredelta{\textbf{3.36}}{+2.15} & \scoredelta{\textbf{4.04}}{+2.78} & \scoredelta{\textbf{2.60}}{+1.56} & \scoredelta{\textbf{3.33}}{+2.16} \\
\tabbodyrule
\multicolumn{5}{@{}>{\hspace{2pt}}l}{\textbf{Bernini-R-14B}} \\
Base & \scoreonly{2.48} & \scoreonly{2.21} & \scoreonly{2.06} & \scoreonly{2.25} \\
\methodname & \scoredelta{\textbf{3.38}}{+0.90} & \scoredelta{\textbf{3.51}}{+1.30} & \scoredelta{\textbf{2.91}}{+0.85} & \scoredelta{\textbf{3.27}}{+1.02} \\
\end{tabular*}
\caption{\textbf{New editing abilities after distillation}. All three students improve on their base editors.}
\label{tab:new}
\end{table}





\begin{table*}[t]
\centering
\newcommand{\tablebasedelta}[1]{{\fontsize{7}{8}\selectfont
  \ifdim #1pt>0pt\textcolor{i2vtgain}{#1}%
  \else\ifdim #1pt<0pt\textcolor{i2vtdrop}{#1}%
  \else #1\fi\fi}}
\newcommand{\tablejudgepair}[2]{#1\kern0.08em/\kern0.08em#2}
\fontsize{8}{9.5}\selectfont
\setlength{\tabcolsep}{1pt}
\begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}>{\hspace{2pt}}lcccccccccccc<{\hspace{2pt}}@{}}
 &  & \multicolumn{6}{c}{\tablehead{OpenVE-Bench (Gemini 2.5 Pro)}} & \multicolumn{5}{c}{\tablehead{\benchname (Gemini 2.5 Pro / 3.8 Flash)\hyperref[fn:gemini-transition]{\textsuperscript{\ref*{fn:gemini-transition}}}}} \\
\tabgrouprule{3-8}\tabgrouprule{9-13}
\tablehead{Model} & \tablehead{Model\\size} & \tablehead{Global\\Style$^{\uparrow}$} & \tablehead{Local\\Change$^{\uparrow}$} & \tablehead{Background\\Change$^{\uparrow}$} & \tablehead{Local\\Remove$^{\uparrow}$} & \tablehead{Local\\Add$^{\uparrow}$} & \tablehead{Overall$^{\uparrow}$} & \tablehead{Action\\Change$^{\uparrow}$} & \tablehead{Expression\\Change$^{\uparrow}$} & \tablehead{Body\\Movement$^{\uparrow}$} & \tablehead{Scene\\Relighting$^{\uparrow}$} & \tablehead{Overall$^{\uparrow}$} \\
\tabheadrule
Bernini-R-1.3B$^\star$~\citep{bernini2026bernini} & 1.3B & 3.27 & 4.01 & 2.94 & 2.88 & 2.41 & 3.10 & \tablejudgepair{1.83}{1.43} & \tablejudgepair{2.00}{1.50} & \tablejudgepair{1.14}{1.10} & \tablejudgepair{2.43}{2.11} & \tablejudgepair{1.85}{1.54} \\
Lucy-Edit~\citep{decart2025lucyedit} & 5B & 2.27 & 3.20 & 1.57 & 1.75 & 2.30 & 2.22 & \tablejudgepair{1.96}{1.34} & \tablejudgepair{2.25}{1.51} & \tablejudgepair{1.08}{1.04} & \tablejudgepair{2.53}{2.07} & \tablejudgepair{1.95}{1.49} \\
OpenVE-Edit~\citep{he2025openve} & 5B & 3.16 & 2.98 & 2.36 & 1.85 & 2.15 & 2.50 & -- & -- & -- & -- & -- \\
Kiwi-Edit~\citep{lin2026kiwiedit} & 5B & 3.72 & 3.91 & 2.67 & 2.69 & 2.55 & 3.11 & \tablejudgepair{2.34}{1.11} & \tablejudgepair{2.65}{1.97} & \tablejudgepair{1.22}{1.00} & \tablejudgepair{2.78}{2.43} & \tablejudgepair{2.25}{1.63} \\
LoomVideo (RL)~\citep{loomvideo2026} & 5B & 3.85 & 3.41 & 2.37 & 3.12 & 2.19 & 2.99 & \tablejudgepair{2.35}{1.26} & \tablejudgepair{2.80}{1.40} & \tablejudgepair{1.37}{1.30} & \tablejudgepair{3.31}{3.10} & \tablejudgepair{2.46}{1.77} \\
ICVE~\citep{liao2025icve} & 13B & 2.22 & 2.57 & 1.62 & 2.51 & 1.97 & 2.18 & \tablejudgepair{1.10}{1.24} & \tablejudgepair{1.18}{1.56} & \tablejudgepair{1.01}{1.07} & \tablejudgepair{1.69}{1.98} & \tablejudgepair{1.24}{1.46} \\
VACE~\citep{jiang2025vace} & 14B & 1.49 & 2.07 & 1.55 & 1.46 & 1.26 & 1.57 & \tablejudgepair{1.75}{1.10} & \tablejudgepair{1.94}{1.36} & \tablejudgepair{1.06}{1.00} & \tablejudgepair{2.27}{2.77} & \tablejudgepair{1.76}{1.56} \\
Ditto~\citep{bai2026ditto} & 14B & 4.01 & 2.03 & 1.68 & 1.53 & 1.41 & 2.13 & \tablejudgepair{1.75}{1.68} & \tablejudgepair{2.14}{2.79} & \tablejudgepair{1.05}{1.00} & \tablejudgepair{2.25}{3.03} & \tablejudgepair{1.80}{2.13} \\
VideoCoF$^\star$~\citep{yang2025videocof} & 14B & 1.31 & 3.59 & 1.55 & 2.48 & 2.50 & 2.29 & \tablejudgepair{1.21}{1.11} & \tablejudgepair{1.26}{1.12} & \tablejudgepair{1.04}{1.00} & \tablejudgepair{1.27}{1.41} & \tablejudgepair{1.20}{1.16} \\
Bernini-R-14B$^\star$~\citep{bernini2026bernini} & 14B & 4.16 & 4.30 & 3.16 & 2.66 & 2.35 & 3.33 & \tablejudgepair{2.48}{2.57} & \tablejudgepair{2.21}{1.31} & \tablejudgepair{2.06}{2.47} & \tablejudgepair{3.02}{2.84} & \tablejudgepair{2.44}{2.30} \\
JoyAI-Video-Edit$^\star$~\citep{xiao2026joyaivideoedit} & 16B & 3.89 & 4.37 & 2.86 & 2.72 & 2.55 & 3.28 & \tablejudgepair{2.74}{2.51} & \tablejudgepair{3.02}{2.21} & \tablejudgepair{2.50}{2.52} & \tablejudgepair{3.79}{3.76} & \tablejudgepair{3.01}{2.75} \\
VInO~\citep{chen2026vino} & 17B & 4.34 & 3.73 & 2.54 & 3.22 & \textbf{2.77} & 3.32 & \tablejudgepair{3.20}{3.29} & \tablejudgepair{3.40}{3.94} & \tablejudgepair{2.21}{2.45} & \tablejudgepair{2.50}{3.55} & \tablejudgepair{2.83}{3.31} \\
\tabbodyrule
\shadedrow
\modelsmall & 1.3B & 3.93 & 4.01 & 3.12 & \textbf{3.45} & 2.59 & 3.42 & \tablejudgepair{\textbf{3.47}}{3.35} & \tablejudgepair{3.47}{3.67} & \tablejudgepair{2.32}{2.90} & \tablejudgepair{3.21}{3.65} & \tablejudgepair{3.12}{3.39} \\
\shadedrow
{\fontsize{7}{8}\selectfont$\Delta$ \textit{vs. Base}} &  & \tablebasedelta{+0.66} & \tablebasedelta{0.00} & \tablebasedelta{+0.18} & \tablebasedelta{+0.57} & \tablebasedelta{+0.18} & \tablebasedelta{+0.32} & \tablejudgepair{\tablebasedelta{+1.64}}{\tablebasedelta{+1.92}} & \tablejudgepair{\tablebasedelta{+1.47}}{\tablebasedelta{+2.17}} & \tablejudgepair{\tablebasedelta{+1.18}}{\tablebasedelta{+1.80}} & \tablejudgepair{\tablebasedelta{+0.78}}{\tablebasedelta{+1.54}} & \tablejudgepair{\tablebasedelta{+1.27}}{\tablebasedelta{+1.85}} \\
\shadedrow
\modellarge & 14B & \textbf{4.45} & \textbf{4.62} & \textbf{3.27} & 3.14 & 2.44 & \textbf{3.58} & \tablejudgepair{3.45}{3.86} & \tablejudgepair{3.41}{3.82} & \tablejudgepair{\textbf{3.02}}{\textbf{3.67}} & \tablejudgepair{3.47}{3.73} & \tablejudgepair{\textbf{3.34}}{3.77} \\
\shadedrow
{\fontsize{7}{8}\selectfont$\Delta$ \textit{vs. Base}} &  & \tablebasedelta{+0.29} & \tablebasedelta{+0.32} & \tablebasedelta{+0.11} & \tablebasedelta{+0.48} & \tablebasedelta{+0.09} & \tablebasedelta{+0.25} & \tablejudgepair{\tablebasedelta{+0.97}}{\tablebasedelta{+1.29}} & \tablejudgepair{\tablebasedelta{+1.20}}{\tablebasedelta{+2.51}} & \tablejudgepair{\tablebasedelta{+0.96}}{\tablebasedelta{+1.20}} & \tablejudgepair{\tablebasedelta{+0.45}}{\tablebasedelta{+0.89}} & \tablejudgepair{\tablebasedelta{+0.90}}{\tablebasedelta{+1.47}} \\
\shadedrow
\modelcof & 14B & 3.51 & 3.81 & 2.81 & 2.96 & 2.54 & 3.13 & \tablejudgepair{3.11}{\textbf{4.07}} & \tablejudgepair{\textbf{3.93}}{\textbf{4.53}} & \tablejudgepair{2.36}{3.14} & \tablejudgepair{\textbf{3.84}}{\textbf{4.27}} & \tablejudgepair{3.31}{\textbf{4.01}} \\
\shadedrow
{\fontsize{7}{8}\selectfont$\Delta$ \textit{vs. Base}} &  & \tablebasedelta{+2.20} & \tablebasedelta{+0.22} & \tablebasedelta{+1.26} & \tablebasedelta{+0.48} & \tablebasedelta{+0.04} & \tablebasedelta{+0.84} & \tablejudgepair{\tablebasedelta{+1.90}}{\tablebasedelta{+2.96}} & \tablejudgepair{\tablebasedelta{+2.67}}{\tablebasedelta{+3.41}} & \tablejudgepair{\tablebasedelta{+1.32}}{\tablebasedelta{+2.14}} & \tablejudgepair{\tablebasedelta{+2.57}}{\tablebasedelta{+2.86}} & \tablejudgepair{\tablebasedelta{+2.11}}{\tablebasedelta{+2.85}} \\
\end{tabular*}
\caption{\textbf{One \methodname model handles both basic edits and new editing tasks.} All scores are reported without prompt enhancement. We cite OpenVE-Bench baselines from previous work except those marked $\star$, and run all \benchname evaluations ourselves.}
\label{tab:main}
\end{table*}

Training on individual images raises the new-task overall score of Bernini-R-1.3B from $1.66$ to $2.99$ and Bernini-R-14B from $2.25$ to $3.27$ (\Cref{tab:new}). VideoCoF gains the most, rising from $1.17$ to $3.33$ and \textbf{reaching a similar level to fine-tuned Bernini-R-14B despite its weaker starting point}. The action and expression edits in \Cref{fig:main_new_abilities} illustrate how the abilities learned from images transfer to video clips.

\subsection{Offline Distillation versus I2VT}
\label{sec:offline_comparison}

To test whether more offline timesteps per image or a larger image batch can match online rollout supervision, we compare offline configurations of $24\times1$, $24\times10$, and $240\times1$ with \methodname, where the factors denote images per update and states per image. We train Bernini-R-1.3B separately on basic and new tasks for 200 updates using the same source images and teacher. The default offline setup samples ten independent noise states per image, matching the ten supervised rollout timesteps in \methodname. Both use 24 images and 240 supervised states per update (\Cref{tab:offline_comparison}).



\begingroup
\setlength{\intextsep}{6pt}
\begin{table}[!htb]
\centering
\fontsize{8}{9.5}\selectfont
\renewcommand{\deltasize}{\fontsize{4.5}{5.5}\selectfont}
\setlength{\tabcolsep}{0.5pt}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}>{\hspace{2pt}}lccccc<{\hspace{2pt}}@{}}
\tablehead[l]{Method} & Base & \multicolumn{3}{c}{Offline} & \methodname \\
\tablehead[l]{Batch size} & -- & $24\times1$ & $24\times10$ & $240\times1$ & $24\times10$ \\
\tabheadrule
\multicolumn{6}{l}{\textbf{OpenVE-Bench: basic edits$^{\uparrow}$}} \\
Global Style & \scoreonly{3.27} & \scoredelta{3.80}{+0.53} & \scoredelta{3.97}{+0.70} & \scoredelta{3.78}{+0.51} & \scoredelta{\textbf{4.04}}{+0.77} \\
Local Change & \scoreonly{4.01} & \scoredelta{3.94}{-0.07} & \scoredelta{4.02}{+0.01} & \scoredelta{3.57}{-0.44} & \scoredelta{\textbf{4.21}}{+0.20} \\
Background Change & \scoreonly{2.94} & \scoredelta{2.88}{-0.06} & \scoredelta{2.70}{-0.24} & \scoredelta{2.75}{-0.19} & \scoredelta{\textbf{3.03}}{+0.09} \\
Local Remove & \scoreonly{2.88} & \scoredelta{2.94}{+0.06} & \scoredelta{2.79}{-0.09} & \scoredelta{2.98}{+0.10} & \scoredelta{\textbf{3.50}}{+0.62} \\
Local Add & \scoreonly{2.41} & \scoredelta{2.33}{-0.08} & \scoredelta{2.50}{+0.09} & \scoredelta{2.33}{-0.08} & \scoredelta{\textbf{2.61}}{+0.20} \\
Overall & \scoreonly{3.10} & \scoredelta{3.18}{+0.08} & \scoredelta{3.19}{+0.09} & \scoredelta{3.08}{-0.02} & \scoredelta{\textbf{3.48}}{+0.38} \\
\tabbodyrule
\multicolumn{6}{l}{\textbf{\benchname: new tasks$^{\uparrow}$}} \\
Action Change & \scoreonly{1.83} & \scoredelta{\textbf{3.26}}{+1.43} & \scoredelta{3.24}{+1.41} & \scoredelta{3.13}{+1.30} & \scoredelta{3.21}{+1.38} \\
Expression Change & \scoreonly{2.00} & \scoredelta{3.08}{+1.08} & \scoredelta{3.10}{+1.10} & \scoredelta{3.07}{+1.07} & \scoredelta{\textbf{3.58}}{+1.58} \\
Body Movement & \scoreonly{1.14} & \scoredelta{1.87}{+0.73} & \scoredelta{1.88}{+0.74} & \scoredelta{\textbf{2.20}}{+1.06} & \scoredelta{2.18}{+1.04} \\
Overall & \scoreonly{1.66} & \scoredelta{2.73}{+1.07} & \scoredelta{2.74}{+1.08} & \scoredelta{2.80}{+1.14} & \scoredelta{\textbf{2.99}}{+1.33} \\
\end{tabular*}
\caption{\textbf{Offline configurations on Bernini-R-1.3B.} Basic and new tasks are trained separately.}
\label{tab:offline_comparison}
\end{table}
\endgroup

\textbf{Offline distillation learns new tasks}, but its basic-edit gains involve trade-offs: all three configurations improve global style while reducing background-change scores. The comparison in \Cref{fig:main_basic_comparison} illustrates a remaining gap on body movement, where the offline model leaves the woman seated while \methodname produces the requested standing pose. Although some offline configurations slightly outperform \methodname on action changes or body movements, \textbf{\methodname achieves the highest overall scores on both task pools}, reaching $3.48$ on basic edits and $2.99$ on new tasks (\Cref{tab:offline_comparison}).





\Needspace{5\baselineskip}
\section{Evaluation}
\label{sec:overall_evaluation}


\subsection{Comparison with Existing Video Editors}
\label{sec:allin}

\begingroup\PaperAvoidWidow
We fine-tune the three base editors on both pools of \datasetfull (\Cref{sec:training_data}) and name the resulting models \modelsmall, \modellarge, and \modelcof. Each model handles both basic and new edits.\par
\endgroup




\Needspace{3\baselineskip}
\textbf{Our models achieve state-of-the-art results} among the compared open-source video editors, with \modellarge scoring $3.58$ on OpenVE-Bench and $3.34$ on \benchname under Gemini 2.5 Pro, and \modelcof scoring $4.01$ on \benchname under Gemini 3.8 Flash.\footnote{\label{fn:gemini-transition}Google will retire Gemini 2.5 Pro from its API on \href{https://ai.google.dev/gemini-api/docs/deprecations\#gemini-2.5-pro-models}{December 1, 2026}, so we also report Gemini 3.8 Flash scores for future comparisons on \benchname. A dash marks an unavailable score.}
Under Gemini 2.5 Pro, jointly fine-tuned models (\Cref{tab:main}) perform close to separately fine-tuned models on the basic edits and three new task groups in \Cref{tab:old,tab:new}.
\Cref{fig:model_comparison} compares \modelsmall with JoyAI-Video-Edit~\citep{xiao2026joyaivideoedit} and LoomVideo (RL)~\citep{loomvideo2026} on action and expression edits.

\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{figures/qualitative_results.pdf}
\caption{\textbf{Qualitative results.} Top and middle rows show new and basic edits, comparing the source, base editor, and \methodname. The bottom row compares \modelsmall with other editors on \benchname action and expression edits. Each video shows two frames at matched times.}
\label{fig:qualitative}
\label{fig:main_new_abilities}
\label{fig:basic_edit_types}
\label{fig:model_comparison}
\end{figure*}



\subsection{Ablation Study}
\label{sec:ablation}

We ablate two design choices in \methodname: the guidance scales that shape supervision and rollout states, and the loss that matches the student prediction to the teacher target. The teacher, student, and rollout scales control the three applications of classifier-free guidance in \Cref{sec:opd}. All ablations use Bernini-R-1.3B with the setup in \Cref{sec:eval_setup}, trained on the OpenVE pool or the three new task groups in \Cref{sec:new}.

\subsubsection{Guidance Scales}
\label{sec:guidance_scales}

On the OpenVE pool, we vary one guidance scale at a time from the default $\omega_R=\omega_S=\omega_T=1$ (\Cref{tab:abl_teacher}). For the new tasks, we compare using $\omega_T=1$ for every task with using $\omega_T=2$ for actions and body movements and $\omega_T=1$ for expressions (\Cref{tab:abl_new}).

\begin{table}[!htb]
\centering
\fontsize{8}{9.5}\selectfont
\renewcommand{\deltasize}{\fontsize{4.5}{5.5}\selectfont}
\setlength{\tabcolsep}{1.6pt}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}>{\hspace{2pt}}lcccccc<{\hspace{2pt}}@{}}
\tablehead{Setting} & \tablehead{Global\\Style$^{\uparrow}$} & \tablehead{Local\\Change$^{\uparrow}$} & \tablehead{Background\\Change$^{\uparrow}$} & \tablehead{Local\\Remove$^{\uparrow}$} & \tablehead{Local\\Add$^{\uparrow}$} & \tablehead{Overall$^{\uparrow}$} \\
\tabheadrule
Base & \scoreonly{3.27} & \scoreonly{4.01} & \scoreonly{2.94} & \scoreonly{2.88} & \scoreonly{2.41} & \scoreonly{3.10} \\
\shadedrow
Default & \scoredelta{\textbf{4.04}}{+0.77} & \scoredelta{\textbf{4.21}}{+0.20} & \scoredelta{\textbf{3.03}}{+0.09} & \scoredelta{\textbf{3.50}}{+0.62} & \scoredelta{2.61}{+0.20} & \scoredelta{\textbf{3.48}}{+0.38} \\
$\omega_R=5$ & \scoredelta{3.83}{+0.56} & \scoredelta{\textbf{4.21}}{+0.20} & \scoredelta{3.02}{+0.08} & \scoredelta{3.16}{+0.28} & \scoredelta{2.55}{+0.14} & \scoredelta{3.35}{+0.25} \\
$\omega_S=2$ & \scoredelta{3.54}{+0.27} & \scoredelta{4.18}{+0.17} & \scoredelta{2.46}{-0.48} & \scoredelta{2.88}{0.00} & \scoredelta{\textbf{2.81}}{+0.40} & \scoredelta{3.17}{+0.07} \\
$\omega_S=5$ & \scoredelta{2.04}{-1.23} & \scoredelta{2.79}{-1.22} & \scoredelta{1.42}{-1.52} & \scoredelta{1.60}{-1.28} & \scoredelta{1.57}{-0.84} & \scoredelta{1.88}{-1.22} \\
$\omega_T=2$ & \scoredelta{3.84}{+0.57} & \scoredelta{4.06}{+0.05} & \scoredelta{2.82}{-0.12} & \scoredelta{3.19}{+0.31} & \scoredelta{2.39}{-0.02} & \scoredelta{3.26}{+0.16} \\
$\omega_T=5$ & \scoredelta{3.70}{+0.43} & \scoredelta{3.98}{-0.03} & \scoredelta{2.64}{-0.30} & \scoredelta{3.24}{+0.36} & \scoredelta{2.47}{+0.06} & \scoredelta{3.20}{+0.10} \\
\end{tabular*}
\caption{\textbf{Ablation on guidance scales.} On OpenVE-Bench, the default $\omega_R=\omega_S=\omega_T=1$ scores highest overall.}
\label{tab:abl_teacher}
\end{table}



On basic edits, \textbf{rollout guidance matters little}: $\omega_R=5$ scores $3.35$ on basic edits, close to the default ($3.48$). In contrast, \textbf{student guidance of $1$ works best among the tested values}: $\omega_S=2$ lowers the score to $3.17$, and $\omega_S=5$ drops it to $1.88$, below Base ($3.10$).

\begin{table}[!htb]
\centering
\fontsize{8}{9.5}\selectfont
\renewcommand{\deltasize}{\fontsize{4.5}{5.5}\selectfont}
\setlength{\tabcolsep}{0.8pt}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}>{\hspace{2pt}}lccccc<{\hspace{2pt}}@{}}
 & \tablehead{Action\\Change$^{\uparrow}$} & \tablehead{Expression\\Change$^{\uparrow}$} & \tablehead{Body\\Movement$^{\uparrow}$} & \tablehead{Overall$^{\uparrow}$} & \tablehead{OpenVE-Bench} \\
\tabheadrule
Base & \scoreonly{1.83} & \scoreonly{2.00} & \scoreonly{1.14} & \scoreonly{1.66} & \scoreonly{3.10} \\
$\omega_T=1$ & \scoredelta{3.01}{+1.18} & \scoredelta{3.57}{+1.57} & \scoredelta{1.99}{+0.85} & \scoredelta{2.86}{+1.20} & \scoredelta{3.12}{+0.02} \\
\shadedrow
$\omega_T=2^{\star}$ & \scoredelta{\textbf{3.21}}{+1.38} & \scoredelta{\textbf{3.58}}{+1.58} & \scoredelta{\textbf{2.18}}{+1.04} & \scoredelta{\textbf{2.99}}{+1.33} & \scoredelta{3.13}{+0.03} \\
\end{tabular*}
\caption{\textbf{Selective teacher guidance.} $\star$: $\omega_T=2$ for actions and body movements, and $\omega_T=1$ for expressions. This setting improves action changes and body movements over using $\omega_T=1$ throughout.}
\label{tab:abl_new}
\end{table}

\textbf{Stronger teacher guidance helps harder tasks.} On basic edits, $\omega_T=2$ and $5$ score $3.26$ and $3.20$, below the default, whereas on the new task groups the selective policy raises the overall score from $2.86$ to $2.99$, with gains in action changes and body movements, and both policies keep the OpenVE-Bench score of Base ($3.12$ and $3.13$ versus $3.10$). 

\begingroup
\setlength{\intextsep}{6pt}
\begin{table}[!t]
\centering
\fontsize{8}{9.5}\selectfont
\renewcommand{\deltasize}{\fontsize{4.5}{5.5}\selectfont}
\setlength{\tabcolsep}{0.8pt}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}>{\hspace{2pt}}lcccccc<{\hspace{2pt}}@{}}
\tablehead{Loss} & \tablehead{Global\\Style$^{\uparrow}$} & \tablehead{Local\\Change$^{\uparrow}$} & \tablehead{Background\\Change$^{\uparrow}$} & \tablehead{Local\\Remove$^{\uparrow}$} & \tablehead{Local\\Add$^{\uparrow}$} & \tablehead{Overall$^{\uparrow}$} \\
\tabheadrule
Base & \scoreonly{3.27} & \scoreonly{4.01} & \scoreonly{2.94} & \scoreonly{2.88} & \scoreonly{2.41} & \scoreonly{3.10} \\
\shadedrow
$\vv$ mse & \scoredelta{\textbf{4.04}}{+0.77} & \scoredelta{\textbf{4.21}}{+0.20} & \scoredelta{\textbf{3.03}}{+0.09} & \scoredelta{\textbf{3.50}}{+0.62} & \scoredelta{2.61}{+0.20} & \scoredelta{\textbf{3.48}}{+0.38} \\
$\vv$ cos & \scoredelta{3.89}{+0.62} & \scoredelta{4.13}{+0.12} & \scoredelta{2.93}{-0.01} & \scoredelta{3.32}{+0.44} & \scoredelta{\textbf{2.65}}{+0.24} & \scoredelta{3.38}{+0.28} \\
$\vx$ mse & \scoredelta{3.86}{+0.59} & \scoredelta{4.16}{+0.15} & \scoredelta{\textbf{3.03}}{+0.09} & \scoredelta{3.47}{+0.59} & \scoredelta{2.44}{+0.03} & \scoredelta{3.39}{+0.29} \\
$\vx$ cos & \scoredelta{3.79}{+0.52} & \scoredelta{4.11}{+0.10} & \scoredelta{3.01}{+0.07} & \scoredelta{3.30}{+0.42} & \scoredelta{2.63}{+0.22} & \scoredelta{3.37}{+0.27} \\
\end{tabular*}
\caption{\textbf{Ablation on matching losses.} We compare velocity ($\vv$) and clean-latent ($\vx$) targets using mean squared error (mse) or cosine distance (cos). All four improve on Base.}
\label{tab:abl_loss}
\end{table}
\endgroup

\subsubsection{Matching Losses}
\label{sec:matching_losses}
Prior on-policy distillation methods match teacher predictions using different formulations~\citep{zhou2026danceopd,li2026diffusionopdunifiedperspectiveonpolicy}. To examine this choice for image-to-video transfer, we compare mean squared error (mse) and cosine distance (cos) on velocity predictions ($\vv$) and predicted clean latents ($\vx$), using the OpenVE pool and $\omega_R=\omega_S=\omega_T=1$ (\Cref{tab:abl_loss}).
Both targets use the same rollout states as in \cref{eq:loss}; teacher targets are detached, and detailed definitions are provided in \PaperSupp{}. Velocity mse scores $3.48$ versus $3.37$--$3.39$ for the other three losses in \Cref{tab:abl_loss}. Both targets improve on Base ($3.10$) with either distance metric.



\subsection{Video Quality and Temporal Quality}
\label{sec:temporal}
To check whether single-frame fine-tuning preserves video and temporal quality while improving editing abilities, we follow VBench~\citep{huang2024vbench} to evaluate \benchname videos edited by \modelsmall, \modellarge, and \modelcof from \Cref{sec:allin}, comparing each with its base editor. We measure subject and background consistency, flickering, motion smoothness, and aesthetic and imaging quality, where higher is better, alongside dynamic degree, which measures motion magnitude.

Temporal and visual scores show small increases and decreases for the Bernini-R series. VideoCoF improves in subject and background consistency as well as aesthetic and imaging quality, with a slight decrease in the flickering score. The editing gains therefore come with \textbf{broadly comparable temporal quality} (\Cref{tab:vbench_openvepp}).

\begin{table}[!htb]
\centering
\fontsize{7}{8.5}\selectfont
\setlength{\tabcolsep}{1.1pt}
\setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}lcccccc@{}}
 & \multicolumn{2}{c}{Bernini-R-1.3B} & \multicolumn{2}{c}{Bernini-R-14B} & \multicolumn{2}{c}{VideoCoF} \\
\tabgrouprule{2-3}\tabgrouprule{4-5}\tabgrouprule{6-7}
 & Base & \methodname & Base & \methodname & Base & \methodname \\
\tabheadrule
Subject cons.$^{\uparrow}$ & 0.9666 & 0.9644 & 0.9603 & 0.9605 & 0.9579 & 0.9707 \\
Background cons.$^{\uparrow}$ & 0.9651 & 0.9625 & 0.9595 & 0.9587 & 0.9563 & 0.9646 \\
Flickering$^{\uparrow}$ & 0.9791 & 0.9793 & 0.9788 & 0.9767 & 0.9826 & 0.9800 \\
Motion smooth.$^{\uparrow}$ & 0.9889 & 0.9894 & 0.9890 & 0.9887 & 0.9901 & 0.9904 \\
Dynamic degree & 0.589 & 0.623 & 0.681 & 0.667 & 0.449 & 0.551 \\
Aesthetic$^{\uparrow}$ & 0.573 & 0.570 & 0.576 & 0.578 & 0.523 & 0.562 \\
Imaging$^{\uparrow}$ & 0.725 & 0.723 & 0.722 & 0.724 & 0.616 & 0.740 \\
\end{tabular*}
\caption{\textbf{Temporal quality remains comparable after fine-tuning.} We report VBench metrics on edited \benchname videos from the base editors and \methodname.}
\label{tab:vbench_openvepp}
\end{table}

\subsection{Out-of-Distribution Generalization}
\label{sec:ivebench}
To test whether the editing gains generalize beyond OpenVE-Bench and \benchname, we evaluate \modelsmall, \modellarge, and \modelcof from \Cref{sec:allin} on the short-video subset of IVEBench~\citep{chen2026ivebench}, whose clips, instructions, and metrics differ from those of OpenVE-Bench.

\begin{table}[!htb]
\centering
\fontsize{7}{8.5}\selectfont
\setlength{\tabcolsep}{0.3pt}
\begin{tabular*}{\linewidth}{@{\extracolsep{\fill}}>{\hspace{2pt}}lcccccc<{\hspace{2pt}}@{}}
 & \tablehead{Overall$^{\uparrow}$} & \tablehead{Instruction\\Compliance$^{\uparrow}$} & \tablehead{Video\\Quality$^{\uparrow}$} & \tablehead{Fidelity$^{\uparrow}$} & \tablehead{Temporal\\Flickering$^{\uparrow}$} & \tablehead{Motion\\Smoothness$^{\uparrow}$} \\
\tabheadrule
VideoCoF & 52.9 & 25.5 & 71.4 & 61.6 & \textbf{96.8} & 97.9 \\
\quad+\,\methodname & \textbf{68.2} & \textbf{40.5} & \textbf{80.6} & \textbf{83.5} & 96.4 & \textbf{98.1} \\
\tabbodyrule
Bernini-R-1.3B & 67.4 & 42.8 & \textbf{79.3} & \textbf{80.2} & 97.7 & \textbf{98.9} \\
\quad+\,\methodname & \textbf{68.9} & \textbf{50.5} & 79.1 & 77.1 & \textbf{97.8} & \textbf{98.9} \\
\tabbodyrule
Bernini-R-14B & 71.0 & 53.7 & \textbf{78.7} & \textbf{80.3} & \textbf{97.8} & \textbf{98.9} \\
\quad+\,\methodname & \textbf{71.5} & \textbf{56.0} & 78.4 & \textbf{80.3} & 97.7 & 98.8 \\
\end{tabular*}
\caption{\textbf{IVEBench results.} \methodname raises the overall score and instruction compliance of all three editors, and temporal quality stays on par with the base editors. Short-video subset, scores $\times100$.}
\label{tab:ivebench_main}
\end{table}

\methodname \textbf{improves instruction compliance and overall scores on this out-of-distribution benchmark} (\Cref{tab:ivebench_main}). VideoCoF shows substantial gains, whereas Bernini-R-1.3B's fidelity falls from $80.2$ to $77.1$, partly offsetting the instruction-compliance gain in Overall, which averages compliance, quality, and fidelity.\footnote{Fidelity measures similarity to the source. The IVEBench authors note that leaving edits incomplete can yield high fidelity; see their \href{https://github.com/RyanChenYN/IVEBench/issues/4}{implementation discussion}.} Further comparisons are provided in \PaperSupp{}.


==> sections/5_conclusion.tex <==


\section{Conclusion}
\label{sec:conclusion}

We introduced \methodname, which transfers image editing capabilities to pretrained video editors using only individual source images, without paired videos or architectural changes. Across three video editors, it improves basic edits and enables new editing tasks, while outperforming offline distillation in matched comparisons. These gains carry over to whole video clips, showing that image editing supervision can improve video editing without new video training pairs.

